Study of Tau Leptons from Top Quark Pairs in ATLAS

Top quark pair decay events resulting in final states containing {\tau} leptons present interesting channels in the search for physics beyond the Standard Model. This document describes the in-progress analyses of two channels, {\tau}+jets and {\tau}+l in tt^{-} decays, for the case of a hadronically decaying {\tau} lepton. The studied events are from 1.03 fb-1 of proton-proton collision data at \surds = 7 TeV recorded by the ATLAS Collaboration at the LHC. The goal of the analysis is to look for deviation from Standard Model expectations. Exclusion limits will be produced for the product of the branching ratios BR(t \rightarrow H+b) and BR(H+ \rightarrow {\tau}{\nu}) with respect to the charged Higgs boson mass, and also on the tan({\beta}) - MH+ plane in the mh-max scenario of the MSSM.

==> 0326743.tex <==
%auto-ignore
